High Performance Computing and Computational Intelligence Applications with MultiChaos Perspective

The experience of the COVID-19 pandemic, which has accelerated many chaotic processes in modern society, has highlighted in a very serious and urgent way the need to understand complex processes in order to achieve the common well-being. Modern High performance computing technologies, Quantum Computing, Computational Intelligence are shown to be extremely efficient and useful in safeguarding the fate of mankind. These technologies are the state of the art of IT evolution and are fundamental to be competitive and efficient today. If a company is familiar with these techniques and technologies, will be able to deal with any unexpected and complicated scenario more efficiently and effectively. The main contribution of our work is a set of best practices and case studies that can help the researcher address computationally complex problems. We offer a range of software technologies, from high performance computing to machine learning and quantum computing, which represent today the state of the art to deal with extremely complex computational issues, driven by chaotic events and not easily predictable. In this chapter we analyse the different technologies and applications that will lead mankind to overcome this difficult moment, as well as to understand more and more deeply the profound aspects of very complex phenomena. In this environment of rising complexity, both in terms of technology, algorithms, and changing lifestyles, it is critical to emphasize the importance of achieving maximum efficiency and outcomes while protecting the integrity of everyone's personal data and respecting the human being as a whole.

==> aboutauthors.tex <==
\begin{frontmatter}
\chapter*{Biography}
\end{frontmatter}

\begin{biography}
\section*{Damiano Perri} 
Damiano Perri is a Ph.D. candidate  in  Computer  Science  in  the  joint  Ph.D. Program  in Mathematics, Statistics and Computer Science between the Departments of Mathematics and Computer Science of the Universities of Florence and University of Perugia, where he also received his BSc degree and MSc summa cum laude.  
His research activity if focused on GPGPU Computing, Parallel and Distributed environments, Virtual and Augmented Reality, Artificial Intelligence, Neural Networks. 
In particular his recent research activity is aimed at investigating predictive models in order to optimise the most important operators in emerging Convolutional Neural Networks (CNNs). 
He is an expert developer of synthetic environments and their applications in everyday life.
Since 2016 he has been the technical manager of the LibreEOL project (\url{https://www.libreeol.org/info}).
In 2020 and in 2021 he was Technology Chair at the International Conference on Computational Science and its Applications (ICCSA).



\section*{Marco Simonetti} 
Marco Simonetti graduated in Electronic Engineering from the University of Bologna, with a thesis on transmission systems with chaotic carrier.

He worked in the Clinical Engineering sector and participated with a work team in the creation of automated systems for Health Administrations. He works as a high school teacher of Mathematics and is currently a PhD student in Computer Science at the University of Florence and affiliation with the University of Perugia. In his interests there are Deep Learning and Neural Networks, Quantum Computing and Didactics of Mathematics.


\section*{Osvaldo Gervasi} 
Osvaldo Gervasi is an Associate Professor in Computer Engineering at the Dept. of Mathematics and Computer Science of Perugia University.
His current research interests include Computational Science, models and algorithms for Distributed Computing, Artificial Intelligence, Cloud Computing, and GPGPU computing, models and algorithms for Virtual and Augmented Reality, and Web information systems modeling and engineering. He wrote more than 120 articles in scientific Journals and Conference Proceedings and co-edited more than 100 books of Proceedings.
He served several times as Invited/Keynote Speaker in International Conferences worldwide. He covers a large number of roles in international journals, such as Editor-In-Chief, Associate Editor, Special Issue Editor (International Journal of Grid and Distributed Computing; Virtual Reality; Transactions on Computational Science; International Journal of Energy, Information and Communications). He covers a large number of roles in international conferences, such as General Chair, Program Chair, Workshop Chair and Publicity Chair. He serves as Review Board Member in a large number of international journals. He is President of the not fpr profit Organization International Conference on Computational Science and Its Applications (ICCSA). He is currently Deputy Director of the Department of Mathematics and Computer Science of Perugia University.



\section*{Sergio Tasso} 
Sergio Tasso is a researcher in Informatics (INF01) at the Department of Mathematics and Computer Science, University of Perugia. He teaches three courses to the students of Informatics: Simulation, Open and Distributed Systems and Computer Networks: Protocols. His research lines are covering the following areas: Simulations of complex systems, Algorithms for molecular science, Multimedia and Internet computing, Web Services and E-learning. He has delivered communications to national and international conferences. He is reviewer and member of the Program Committee of The International Conference on Computational Science and Its Applications (ICCSA).

\end{biography}


==> contributors.tex <==
%% Contributors list %%
\begin{frontmatter}
\chapter*{Contributors}
\end{frontmatter}

\begin{contributorslist}

\end{contributorslist}



==> dedication.tex <==
  %% Dedication page
\begin{dedication}
  %% Dedication
  %% can be few\\
  %% lines long
\end{dedication}


==> listoffigures.tex <==
\begin{frontmatter}
\chapter*{List of Figures}
\end{frontmatter}

\listoffigures


==> part.tex <==
\cleardoublepage
\begin{frontmatter}
%\part{}
\end{frontmatter}

% Text ...


==> part1.tex <==
\begin{frontmatter}
\part{Part title}\label{part1}
\end{frontmatter}

% Text ...


==> preface.tex <==
\cleardoublepage
\begin{frontmatter}
\chapter*{Preface}%
%\addcontentsline{toc}{schapter}{Preface}
\end{frontmatter}


 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

\source%
{%
  \author{Name}\\%
  % \address{Location}\\%
  % \date{Month Year}%
}


==> references.tex <==
%\begin{frontmatter}
%  \chapter*{References}
%  \markboth{References}{References}
%\end{frontmatter}

\begin{thebibliography}{10}

% \bibitem{..}
% \bibitem[]{..}

\end{thebibliography}

==> tableofcontents.tex <==
%% Table of Contents %%
\begin{frontmatter}
\chapter*{Contents}
\end{frontmatter}

\tableofcontents


==> titlepage.tex <==
%% Title Page %%
\begin{titlepage}%
  \begin{titlepagerule}
    \title{Multi-chaos, Fractal and Multi-fractional AI of Different Complex Systems}
    \subtitle{Via Theory, Complex Paradoxical Analyses and Harmonic Analysis: Beyond Reliable Global Optimal Solutions based on Mathematical Modelling}
    %\volume{2}
  \end{titlepagerule}

  \edition{2nd edition}

%  \editedby{Edited by}

  \author{Yeliz Karaca}
  \address{University of Massachusetts Medical School, Worcester,
MA 01655, USA, e-mail: yeliz.karaca@ieee.org}

  \author{Dumitru Baleanu}
  \address{Department of Mathematics, Faculty of Art and Sciences, Çankaya University, Ankara, Turkey and Institute of Space
Sciences,Magurele-Bucharest,Romania,e-mail:dumitru@cankaya.edu.tr}

\author{Yu-Dong Zhang}
\address{Department of Informatics, University of Leicester,
Leicester, LE1 7RH, United Kingdom, e-mail: yudongzhang@ieee.org}

\author{Khan Muhammad} 
\address{Department of Software, Sejong University, Seoul,
South Korea, e-mail: khan@sejong.ac.kr}
  
\author{Osvaldo Gervasi}
\address{University of Perugia, Department of Mathematics and Computer Science, Perugia, Italy, email:osvaldo.gervasi@unipg.it}  
  
  \author{Majaz Moonis}
\address{University of Massachusetts Medical School, Worcester, MA 01655,USA, e-mail: Majaz.Moonis@umassmemorial.org)}

  
  
\end{titlepage}

